Electroweak Radiative Corrections for Collider Physics

Current particle phenomenology is characterized by the spectacular agreement of the predictions of the Standard Model of particle physics (SM) with all results from collider experiments and by the absence of significant signals of non-standard physics, despite the fact that we know that the SM cannot be the ultimate theory of nature. In this situation, confronting theory and experiment with high precision is a promising direction to look for potential traces of physics beyond the SM. On the theory side, the calculation of radiative corrections of the strong and electroweak interactions is at the heart of this task, a field that has seen tremendous conceptual and technical progress in the last decades. This review aims at a coherent introduction to the field of electroweak corrections and tries to fill gaps in the literature between standard textbook knowledge and the current state of the art. The SM and the machinery for its perturbative evaluation are reviewed in detail, putting particular emphasis on renormalization, on one-loop techniques, on modern amplitude methods and tools, on the separation of infrared singularities in real-emission corrections, on electroweak issues connected with hadronic initial or final states in collisions, and on the issue of unstable particles in quantum field theory together with corresponding practical solutions.

==> newcommands.tex <==
% relax positioning of floats
\renewcommand{\topfraction}{1}
\renewcommand{\bottomfraction}{1}
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}    
\renewcommand{\textfraction}{0.07}
\renewcommand{\floatpagefraction}{0.9}

% remove widows and clubs
\displaywidowpenalty=10000
\clubpenalty=10000
\widowpenalty=10000

\hfuzz 1pt

% hyphenation patterns
\hyphenation{brems-strah-lung coun-ter-terms La-gran-gi-an}

% allow breaks in multiline equations
\RequirePackage{amsmath}
\allowdisplaybreaks

% comments
\newcommand{\SDcomment}[1]{{\color{red} #1}}
\newcommand{\ADcomment}[1]{{\color{blue} #1}}

%  Abbreviations and math space and characters
\RequirePackage{xspace}
\providecommand*\eg{e.g.\@\xspace}
\providecommand*\ie{i.e.\@\xspace}
\providecommand*\cf{cf.\@\xspace}
\providecommand*\etc{etc.\@\xspace}
\providecommand*\etal{et al.\@\xspace}

% roman letters for mathematical constants and operators
\providecommand{\rd}{\ensuremath{\mathrm{d}}}
\providecommand{\re}{\ensuremath{\mathrm{e}}}
\providecommand{\rE}{\ensuremath{\mathrm{E}}}
\providecommand{\ri}{\ensuremath{\mathrm{i}}}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}
\providecommand{\hc}{\ensuremath{\text{h.c.}}\xspace}

% mathematical objects 
%\newcommand{\order}[1]{\ensuremath{\mathcal{O}{\left(#1\right)}}\xspace}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}{(#1)}}\xspace}
\let\gsim\gtrsim
\let\lsim\lesssim
\makeatletter
\def\asymp#1%
{\mathrel{\raisebox{-.4em}{$\widetilde{\scriptstyle #1}$}}}
%\newcommand{\dsl}[1]{\not \hspace{-0.7mm}#1}
\def\Nlim#1{\mathrel{\raisebox{-.4em}
{$\stackrel{\displaystyle\longrightarrow}{\scriptstyle#1}$}}}
\def\dsl{\mathpalette\make@slash}
\def\make@slash#1#2{\setbox\z@\hbox{$#1#2$}%
  \hbox to 0pt{\hss$#1/$\hss\kern-\wd0}\box0}
\makeatother
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\sumbar}{\mathop{\overline{\sum}}}

% Names for structural elements and references to them
% At beginning of sentence Figure, Equation, Reference should be spelled out
\RequirePackage{ifthen}
\providecommand*{\Eq}[1][s]{\ifthenelse{\equal{#1}{b}}{Equation}{Eq.}}
\providecommand*{\Eqs}[1][s]{\ifthenelse{\equal{#1}{b}}{Equations}{Eqs.}}
\providecommand*{\Figure}[1][s]{\ifthenelse
                                      {\equal{#1}{b}}{Figure}{Fig.}}
\providecommand*{\Figures}[1][s]{\ifthenelse
                                      {\equal{#1}{b}}{Figures}{Figs.}}
\providecommand*{\Ref}[1][s]{\ifthenelse{\equal{#1}{b}}{Reference}{Ref.}}
\providecommand*{\Refs}[1][s]{\ifthenelse{\equal{#1}{b}}{References}{Refs.}}
\providecommand\Table{Table}
\providecommand\Tables{Tables}
\providecommand\Chapter{Chapter}
\providecommand\Chapters{Chapters}
\providecommand\Section{Section}
\providecommand\Sections{Sections}
\providecommand\Appendix{Appendix}
\providecommand\Appendices{Appendices}
\providecommand*\Bref[2][s]{\Ref[#1]~\cite{#2}}
\providecommand*\Brefs[2][s]{\Refs[#1]~\cite{#2}}
\providecommand*\Eref[2][s]{\Eq[#1]~(\ref{#2})}
\providecommand*\Erefs[2][s]{\Eqs[#1]~(\ref{#2})}
\providecommand*\Fref[2][s]{\Figure[#1]~\ref{#2}}
\providecommand*\Frefs[2][s]{\Figures[#1]~\ref{#2}}
\providecommand*\Sref[1]{\Section~\ref{#1}}
\providecommand*\Srefs[1]{\Sections~\ref{#1}}
\providecommand*\Tref[1]{\Table~\ref{#1}}
\providecommand*\Trefs[1]{\Tables~\ref{#1}}
\providecommand*\Cref[1]{\Chapter~\ref{#1}}
\providecommand*\Crefs[1]{\Chapters~\ref{#1}}
\let\citere\Bref
\let\citeres\Brefs
\let\refeq\Eref
\let\refeqs\Erefs
\providecommand*\refeqf[1]{(\ref{#1})}
\let\refse\Sref
\let\refses\Srefs
\let\refcha\Cref
\let\refchas\Crefs
\let\reffi\Fref
\let\reffis\Frefs
\let\refta\Tref
\let\reftas\Trefs
%\providecommand*\refapp[1]{\Appendix~\ref{#1}}
%\providecommand*\refapps[1]{\Appendices~\ref{#1}}
\providecommand*\refapp[1]{\ref{#1}}
\def\nn{\nonumber}

% shorthand for environments
\newcommand\nl{\notag\\}
\newcommand*\beq{\begin{equation}}
\newcommand*\eeq{\end{equation}}
\newcommand*\beqar{\begin{eqnarray}}
\newcommand*\eeqar{\end{eqnarray}}
\newcommand*\barr{\begin{array}}
\newcommand*\earr{\end{array}}
\newcommand*\bfi{\begin{figure}}
\newcommand*\efi{\end{figure}}
\newcommand*\btab{\begin{table}}
\newcommand*\etab{\end{table}}
\newcommand*\bpm{\begin{pmatrix}}
\newcommand*\epm{\end{pmatrix}}

%Shorthands for Greek letters
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand\eps{\epsilon}
\newcommand\veps{\varepsilon}
\newcommand\la{\lambda}
\newcommand\om{\omega}
\newcommand{\si}{\sigma}
\newcommand{\De}{\Delta}
\newcommand{\Ga}{\Gamma}
\newcommand\La{\Lambda}
\newcommand{\Si}{\Sigma}

% Units
\providecommand*\USP{\,}
\newcommand*{\Unit}[2]{\ensuremath{#1\USP\text{#2}}}
\newcommand{\pba}{\unskip\,\mathrm{pb}}
\newcommand{\fb}{{\ensuremath\unskip\USP\text{fb}}\xspace}
\newcommand{\MeV}{\ensuremath{\unskip\USP\text{Me\kern -0.1em V}}\xspace}
\newcommand{\GeV}{\ensuremath{\unskip\USP\text{Ge\kern -0.1em V}}\xspace}
\newcommand{\TeV}{\ensuremath{\unskip\USP\text{Te\kern -0.1em V}}\xspace}

% delta function
\newcommand{\deuf}{{\de^{(4)}}}


% SM parameters
\newcommand{\GF}{\ensuremath{G_\mu}}
\newcommand{\rs}{{\mathrm{s}}}
\newcommand{\rw}{{\mathrm{w}}}
\newcommand{\sw}{s_{\rw}}
\newcommand{\cw}{c_{\rw}}
\newcommand{\gs}{\ensuremath{g_\mathrm{s}}\xspace}
\newcommand{\alphas}{\ensuremath{\alpha_\rs}\xspace}
\newcommand{\Dalphahad}{\ensuremath{\Delta\alpha^{(5)}_{\mathrm{had}}\xspace}}
\newcommand{\If}{\ensuremath {I_{\rw,\Pf}^3}}
\newcommand{\Qf}{\ensuremath {Q_\Pf}}
\newcommand{\Qq}{\ensuremath {Q_\Pq}}
\newcommand{\Ql}{\ensuremath {Q_\Pl}}
\newcommand{\Qt}{\ensuremath {Q_\Pt}}
\newcommand{\VKM}{\ensuremath {{V}}}
\newcommand{\CL}{C_{\rL}}
\newcommand{\CR}{C_{\rR}}
\newcommand{\NCf}{\mathswitch {N_{\mathrm{C}}^\Pf}}
\newcommand{\NCt}{\mathswitch {N_{\mathrm{C}}^\Pt}}
\newcommand{\NCl}{\mathswitch {N_{\mathrm{C}}^\Pl}}
\newcommand{\NCq}{\mathswitch {N_{\mathrm{C}}^\Pq}}
\newcommand{\alphams}{\hat{\alpha}}
\newcommand{\Zms}{\hat{Z}}
\newcommand{\ems}{\hat{e}}
\newcommand{\gms}{\hat{g}}
\newcommand{\swms}{\hat{s}_{\rw}}
\newcommand{\cwms}{\hat{c}_{\rw}}
\newcommand{\kappams}{\hat{\kappa}}

% Particles
\newcommand{\Pg}{\ensuremath{\mathrm{g}}\xspace}
\newcommand{\PA}{\ensuremath{\gamma}\xspace}
\newcommand{\PW}{\ensuremath{\text{W}}\xspace}
\newcommand{\PWp}{\ensuremath{\PW^+}\xspace}
\newcommand{\PWm}{\ensuremath{\PW^-}\xspace}
\newcommand{\PWpm}{\ensuremath{\PW^\pm}\xspace}
\newcommand{\PZ}{\ensuremath{\text{Z}}\xspace}
\newcommand{\PH}{\ensuremath{\text{H}}\xspace}
\newcommand{\Pe}{\ensuremath{\text{e}}\xspace}
\newcommand{\Pep}{\ensuremath{\Pe^+}\xspace}
\newcommand{\Pem}{\ensuremath{\Pe^-}\xspace}
\newcommand{\Pm}{\ensuremath{\mu}\xspace}
\newcommand{\Pb}{\ensuremath{\text{b}}\xspace}
\newcommand{\Pt}{\ensuremath{\text{t}}\xspace}
\newcommand{\Pu}{\ensuremath{\text{u}}\xspace}
\newcommand{\Pd}{\ensuremath{\text{d}}\xspace}
\newcommand{\Ps}{\ensuremath{\text{s}}\xspace}
\newcommand{\Pc}{\ensuremath{\text{c}}\xspace}
\newcommand{\Pbj}{\ensuremath{\text{j_b}}\xspace}
\newcommand{\Pj}{\ensuremath{\text{j}}\xspace}
\newcommand{\Pp}{\ensuremath{\text{p}}\xspace}
\newcommand{\Pq}{\ensuremath{q}\xspace}
\newcommand{\Pl}{\ensuremath{l}\xspace}
\newcommand{\Pn}{\ensuremath{\nu}\xspace}
\newcommand{\Pne}{\ensuremath{\nu_{\Pe}}\xspace}
\newcommand{\Pf}{\ensuremath{f}\xspace}
           
% Particle masses and widths
\def\mathswitch#1{\relax\ifmmode#1\else$#1$\fi}
%\newcommand{\MWOS}{\ensuremath{M_\PW^\text{OS}}\xspace}
%\newcommand{\MZOS}{\ensuremath{M_\PZ^\text{OS}}\xspace}
\newcommand{\MWOS}{\ensuremath{M_{\PW,\text{OS}}}\xspace}
\newcommand{\MZOS}{\ensuremath{M_{\PZ,\text{OS}}}\xspace}
\newcommand{\Ml}{\ensuremath{m_\Pl}\xspace}
\newcommand{\Me}{\ensuremath{m_\Pe}\xspace}
\newcommand{\MW}{\ensuremath{M_\PW}\xspace}
\newcommand{\MZ}{\ensuremath{M_\PZ}\xspace}
\newcommand{\MH}{\ensuremath{M_\PH}\xspace}
\newcommand{\Mt}{\ensuremath{m_\Pt}\xspace}
\newcommand{\Mb}{\ensuremath{m_\Pb}\xspace}
\newcommand{\Mf}{\ensuremath{m_\Pf}\xspace}
\newcommand{\Mq}{\ensuremath{m_\Pq}\xspace}
\newcommand{\MP}{\ensuremath{M_P}\xspace}
\newcommand{\GP}{\ensuremath{\Gamma_P}\xspace}
\newcommand{\MV}{\ensuremath{M_V}\xspace}
\newcommand{\GV}{\ensuremath{\Gamma_V}\xspace}
\newcommand{\MPOS}{\ensuremath{M_{P,\,\OS}}\xspace}
\newcommand{\GPOS}{\ensuremath{\Gamma_{P,\OS}}\xspace}
\newcommand{\MVOS}{\ensuremath{M_{V,\OS}}\xspace}
\newcommand{\GVOS}{\ensuremath{\Gamma_{V,\OS}}\xspace}

% Particle widths
\newcommand{\GWOS}{\ensuremath{\Gamma_\PW^\text{OS}}\xspace}
\newcommand{\GZOS}{\ensuremath{\Gamma_\PZ^\text{OS}}\xspace}
\newcommand{\GZ}{\ensuremath{\Gamma_\PZ}\xspace}
\newcommand{\GW}{\ensuremath{\Gamma_\PW}\xspace}
\newcommand{\GH}{\ensuremath{\Gamma_\PH}\xspace}
\newcommand{\Gt}{\ensuremath{\Gamma_\Pt}\xspace}

%Fields
\newcommand{\FG}{\ensuremath{G}\xspace}
\newcommand{\FB}{\ensuremath{B}\xspace}
\newcommand{\FW}{\ensuremath{W}\xspace}
\newcommand{\FWp}{\ensuremath{\FW^+}\xspace}
\newcommand{\FWm}{\ensuremath{\FW^-}\xspace}
\newcommand{\FWpm}{\ensuremath{\FW^\pm}\xspace}
\newcommand{\FWmp}{\ensuremath{\FW^\mp}\xspace}
\newcommand{\FZ}{\ensuremath{Z}\xspace}
\newcommand{\FA}{\ensuremath{A}\xspace}
\newcommand{\FH}{\ensuremath{H}\xspace}
\newcommand{\Fe}{\ensuremath{e}\xspace}
\newcommand{\Febar}{\ensuremath{\mathswitch{\bar e}}\xspace}
\newcommand{\Fnu}{\ensuremath{\nu}\xspace}
\newcommand{\Fnubar}{\ensuremath{\bar\nu}\xspace}
\newcommand{\Fne}{\ensuremath{\nu_{\Fe}}\xspace}
\newcommand{\Fd}{\ensuremath{d}\xspace}
\newcommand{\Fu}{\ensuremath{u}\xspace}
\newcommand{\Fs}{\ensuremath{s}\xspace}
\newcommand{\Fc}{\ensuremath{c}\xspace}
\newcommand{\Fb}{\ensuremath{b}\xspace}
\newcommand{\Ft}{\ensuremath{t}\xspace}
\newcommand{\Ftbar}{\ensuremath{\bar t}\xspace}
\newcommand{\FL}{\ensuremath{L}\xspace}
\newcommand{\FQ}{\ensuremath{Q}\xspace}
\newcommand{\FF}{\ensuremath{F}\xspace}
\newcommand{\Fl}{\ensuremath{l}\xspace}
\newcommand{\Flbar}{\ensuremath{\bar{l}}\xspace}
\newcommand{\Fq}{\ensuremath{q}\xspace}
\newcommand{\Ff}{\ensuremath{f}\xspace}
\newcommand{\Fubar}{\ensuremath{\bar u}\xspace}
\newcommand{\Fdbar}{\ensuremath{\bar d}\xspace}
\newcommand{\FQbar}{\ensuremath{\bar Q}\xspace}
\newcommand{\FLbar}{\ensuremath{\bar L}\xspace}
\newcommand{\Ffbar}{\ensuremath{\bar f}\xspace}
\newcommand{\Fqbar}{\ensuremath{\bar q}\xspace}
\newcommand{\FV}{\ensuremath{V}\xspace}
\newcommand{\FVbar}{\ensuremath{\bar{V}}\xspace}
\newcommand{\FS}{\ensuremath{S}\xspace}
\newcommand{\FFbar}{\ensuremath{\bar{F}}\xspace}
\newcommand{\FUbar}{\ensuremath{\bar{U}}\xspace}
\newcommand{\FU}{\ensuremath{{U}}\xspace}

\newcommand{\Gammahat}{\ensuremath{\hat{\Gamma}}\xspace}
\newcommand{\GaBFM}{\ensuremath{\hat{\Gamma}}\xspace}
\newcommand{\Psihat}{\ensuremath{\hat{\Psi}}\xspace}
\newcommand{\Phihat}{\ensuremath{\hat{\Phi}}\xspace}
\newcommand{\FBhat}{\ensuremath{\hat B}\xspace}
\newcommand{\FWhat}{\ensuremath{\hat W}\xspace}
\newcommand{\FWpmhat}{\ensuremath{\hat W^\pm}\xspace}
\newcommand{\FWmphat}{\ensuremath{\hat W^\mp}\xspace}
\newcommand{\FZhat}{\ensuremath{\hat Z}\xspace}
\newcommand{\FAhat}{\ensuremath{\hat A}\xspace}
\newcommand{\FHhat}{\ensuremath{\hat \FH}\xspace}
\newcommand{\Dhat}{\ensuremath{\hat D}\xspace}
\newcommand{\psihat}{\ensuremath{\hat{\psi}}\xspace}
%\newcommand{\Shat}{\ensuremath{\hat S}\xspace}
\newcommand{\phihat}{\ensuremath{\hat \phi}\xspace}
\newcommand{\phipmhat}{\ensuremath{\hat \phi^\pm}\xspace}
\newcommand{\phimphat}{\ensuremath{\hat \phi^\mp}\xspace}
\newcommand{\chihat}{\ensuremath{\hat \chi}\xspace}
\newcommand{\Jhat}{\ensuremath{\hat J}\xspace}
%\newcommand{\Vhat}{\ensuremath{\hat V}\xspace}
\newcommand{\FVhat}{\ensuremath{\hat V}\xspace}
\newcommand{\FShat}{\ensuremath{\hat S}\xspace}
\newcommand{\xihat}{\ensuremath{\hat \xi}\xspace}
\newcommand{\thetahat}{\ensuremath{\hat \theta}\xspace}
\newcommand{\xiQ}{\ensuremath{\xi}\xspace}
\newcommand{\FGhat}{\ensuremath{\hat \FG}\xspace}

\newcommand{\FGn}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\FBn}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\FWn}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\FZn}{\ensuremath{\mathcal{Z}}\xspace}
\newcommand{\FAn}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\gen}{\ensuremath{\bar{e}}\xspace}
\newcommand{\gn}{\ensuremath{\bar{g}}\xspace}
\newcommand{\thetawn}{\ensuremath{\bar{\theta}_\rw}\xspace}
\newcommand{\swn}{\ensuremath{\bar{s}_\rw}\xspace}
\newcommand{\cwn}{\ensuremath{\bar{c}_\rw}\xspace}
\newcommand{\Gn}{\ensuremath{\bar{G}}\xspace}
\let\FHn\FH
\let\phinn\chi
\let\phicn\phi

\newcommand{\FHs}{\ensuremath{\FH'}\xspace}

% sources
\newcommand{\KA}{K_A}
\newcommand{\KV}{K_V}
\newcommand{\KW}{K_W}
\newcommand{\Ku}{K_u}
\newcommand{\Kphi}{K_\phi}
\newcommand{\Kchi}{K_\chi}
\newcommand{\KH}{K_\FH}
\newcommand{\Kpsi}{K_\psi}
\newcommand{\Kpsibar}{K_{\psibar}}
\newcommand{\Kf}{K_\Ff}
\newcommand{\Kfbar}{K_{\Ffbar}}
\newcommand{\KF}{K_\FF}
\newcommand{\KFbar}{K_{\FFbar}}

% barred symbols
\makeatletter
\def\longbar{\mathpalette\make@longbar}
\def\make@longbar#1#2{\setbox\z@\hbox{$#1\mkern-2mu#2\mkern-2mu$}%
  {\mkern2mu\overline{\box0}\mkern2mu}}
\makeatother
\def\phibar{\longbar{\phi}}
\def\Phibar{\longbar{\Phi}}
\def\psibar{\longbar{\psi}}
\def\Psibar{\longbar{\Psi}}
\def\chibar{\longbar{\chi}}
\def\etabar{\bar{\eta}}
\def\ubar{\bar{u}}
\def\vbar{\bar{\varv}}
\def\pbar{\bar{p}}
\newcommand{\dbar}{\bar d \mkern2mu}
\newcommand{\lbar}{\bar l \mkern2mu}

% bare quantities
\newcommand{\MWb}{M_{0,\PW}}
\newcommand{\MZb}{M_{0,\PZ}}
\newcommand{\MHb}{M_{0,\PH}}
\newcommand{\Mfb}{m_{0,\Pf}}
\newcommand{\swb}{s_{0,\rw}}

% shorthands for tadpoles
\newcommand{\dtFJ}{\delta t_{\text{FJTS}}}
\newcommand{\dtPR}{\delta t_{\text{PRTS}}}

% shorthands for self energies
\newcommand{\PIA}{\Pi^{\FA\FA}}
\let\PIAA\PIA
\newcommand{\PIAZ}{\Pi^{\FA\FZ}}
\newcommand{\PIZ}{\Pi^{\FZ\FZ}}
\newcommand{\PIW}{\Pi^{\FW\FW}}
\newcommand{\SIA}{{\Sigma^{\FA\FA}_{\rT}}}
\let\SIAA\SIA
\newcommand{\SIAZ}{{\Sigma^{\FA\FZ}_{\rT}}}
\newcommand{\SIZ}{{\Sigma^{\FZ\FZ}_{\rT}}}
\newcommand{\SIZZ}{\SIZ}
\newcommand{\SIW}{{\Sigma^{\FW}_{\rT}}}
\newcommand{\SIWW}{{\Sigma^{\FW\FW}_{\rT}}}
\newcommand{\SIH}{{\Sigma^{\FH}}}
\newcommand{\PIRA}{{\Pi^{\FA\FA}_{\ren}}}
\newcommand{\PIRAZ}{{\Pi^{\FA\FZ}_{\ren}}}
\newcommand{\PIRZ}{{\Pi^{\FZ\FZ}_{\ren}}}
\newcommand{\PIRW}{{\Pi^{\FW\FW}_{\ren}}}
\newcommand{\SIRA}{{\Sigma^{\FA\FA}_{\ren,\rT}}}
\newcommand{\SIRAZ}{{\Sigma^{\FA\FZ}_{\ren,\rT}}}
\newcommand{\SIRZ}{{\Sigma^{\FZ\FZ}_{\ren,\rT}}}
\newcommand{\SIRW}{{\Sigma^{\FW}_{\ren,\rT}}}
\newcommand{\SIRH}{{\Sigma^{\FH}_{\ren}}}

% shorthands for renormalization constants
\newcommand{\DMWS}{\delta\MW^2}
\newcommand{\DMZS}{\delta\MZ^2}
\newcommand{\DMHS}{\delta\MH^2}
\newcommand{\DZA}{\delta Z_{\FA\FA}}
\newcommand{\DZAZ}{\delta Z_{\FA\FZ}}
\newcommand{\DZZA}{\delta Z_{\FZ\FA}}
\newcommand{\DZZ}{\delta Z_{\FZ\FZ}}
\newcommand{\DZW}{\delta Z_{\FW}}
\newcommand{\DZH}{\delta Z_{\FH}}
\newcommand{\DZesi}{\delta Z^{e,\sigma}}
\newcommand{\DZeL}{\delta Z^{\Fe,\rL}}
\newcommand{\DZeR}{\delta Z^{\Fe,\rR}}
\newcommand{\DZmuL}{\delta Z^{\mu,\rL}}
\newcommand{\DZneL}{\delta Z^{\Fne,\rL}}
\newcommand{\DZnmL}{\delta Z^{\Fnm,\rL}}
\newcommand{\DZfL}{\delta Z^{\Ff,\rL}}
\newcommand{\DZfR}{\delta Z^{\Ff,\rR}}
\newcommand{\DZfLd}{\delta Z^{\Ff,\rL\dagger}}
\newcommand{\DZfRd}{\delta Z^{\Ff,\rR\dagger}}
\newcommand{\DZuL}{\delta Z^{\Fu,\rL}}
\newcommand{\DZuR}{\delta Z^{\Fu,\rR}}
\newcommand{\DZuLd}{\delta Z^{\Fu,\rL\dagger}}
\newcommand{\DZuRd}{\delta Z^{\Fu,\rR\dagger}}
\newcommand{\DZdL}{\delta Z^{\Fd,\rL}}
\newcommand{\DZdR}{\delta Z^{\Fd,\rR}}
\newcommand{\DZdLd}{\delta Z^{\Fd,\rL\dagger}}
\newcommand{\DZdRd}{\delta Z^{\Fd,\rR\dagger}}
\newcommand{\DZlL}{\delta Z^{\Fl,\rL}}
\newcommand{\DZlR}{\delta Z^{\Fl,\rR}}
\newcommand{\DZlLd}{\delta Z^{\Fl,\rL\dagger}}
\newcommand{\DZlRd}{\delta Z^{\Fl,\rR\dagger}}
\newcommand{\DZnL}{\delta Z^{\nu,\rL}}
\newcommand{\DZnR}{\delta Z^{\nu,\rR}}
\newcommand{\DZnLd}{\delta Z^{\nu,\rL\dagger}}
\newcommand{\DZnRd}{\delta Z^{\nu,\rR\dagger}}
\newcommand{\DZe}{\delta Z_{e}}

\newcommand{\DZG}{\delta Z_{\FG}}
\newcommand{\DZq}{\delta Z_{\Fq}}
\newcommand{\DZgs}{\delta Z_{\gs}}

\newcommand{\ren}{\mathrm{R}}
\newcommand{\rRe}{\mathop{\widetilde{\mathrm{Re}}}\nolimits}
\newcommand{\muR}{\mu_\mathrm{R}}
\newcommand{\muF}{\mu_\mathrm{F}}
\newcommand{\muIR}{\mu_\mathrm{IR}}
\newcommand{\deltaDR}{\eps}
\newcommand{\DR}{\mathrm{DR}}
\newcommand{\MR}{\mathrm{MR}}

% various shorthands
\newcommand{\PD}{D}            %  propagator denominator
\newcommand{\PDs}{\tilde{\PD}} %  propagator denominator with shifted momentum
\newcommand{\Pff}{P_{ff}}      %  P_ff splitting function
\newcommand{\Pffunreg}{\hat P_{ff}}   %  unreg. P_ff splitting function


% calligraphic symbols
\newcommand{\cA}{\ensuremath{\mathcal{A}}\xspace}
%\newcommand{\cB}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\cC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\cI}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\cK}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\cL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\cM}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\cN}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\cO}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\cP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\cV}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\cW}{\ensuremath{\mathcal{W}}\xspace}

\newcommand{\ord}{\mathswitch{{\cal{O}}}}
\newcommand{\Oa}{\mathswitch{{\cal{O}}(\alpha)}}
\newcommand{\Oaa}{\mathswitch{{\cal{O}}(\alpha^2)}}
\newcommand{\Oaaa}{\mathswitch{{\cal{O}}(\alpha^3)}}

% roman symbols
\newcommand{\rc}{\ensuremath{\text{c}}\xspace}
\newcommand{\rT}{\ensuremath{\text{T}}\xspace}
\newcommand{\rL}{\ensuremath{\text{L}}\xspace}
\newcommand{\rR}{\ensuremath{\text{R}}\xspace}
\newcommand{\rS}{\ensuremath{\text{S}}\xspace}
\newcommand{\rA}{\ensuremath{\text{A}}\xspace}
\newcommand{\rV}{\ensuremath{\text{V}}\xspace}
\newcommand{\rr}{\ensuremath{\text{r}}\xspace}
\newcommand{\rl}{\ensuremath{\text{l}}\xspace}
\newcommand{\rB}{\ensuremath{\text{B}}\xspace}
\newcommand{\rI}{\ensuremath{\text{I}}\xspace}

\newcommand{\sv}{\ensuremath{\sl v}}

%acronyms
\newcommand{\OS}{{\mathrm{OS}}}
\newcommand{\SU}{{\mathrm{SU}}}
\newcommand{\U}{{\mathrm{U}}}
\newcommand{\QED}{{\mathrm{QED}}}
\newcommand{\QCD}{{\mathrm{QCD}}}
\newcommand{\GSW}{{\mathrm{GSW}}}
\newcommand{\SM}{SM\xspace}
\newcommand{\THDM}{THDM\xspace}
\newcommand{\HSESM}{HSESM\xspace}
\newcommand{\MSSM}{MSSM\xspace}
\newcommand{\MSbar}{\ensuremath{\overline{{\text{MS}}\xspace}}}
\newcommand{\UV}{{\mathrm{UV}}}
\newcommand{\weak}{{\mathrm{weak}}}
\newcommand{\virt}{{\mathrm{virt}}}
\newcommand{\coll}{{\mathrm{coll}}}
\newcommand{\collCT}{{\textrm{coll-ct}}}
\newcommand{\hard}{{\mathrm{hard}}}
\newcommand{\soft}{{\mathrm{soft}}}
\newcommand{\EPA}{{\mathrm{EPA}}}
\newcommand{\ISR}{{\mathrm{ISR}}}
\newcommand{\FSR}{{\mathrm{FSR}}}
\newcommand{\LL}{{\mathrm{LL}}}
\newcommand{\LO}{{\mathrm{LO}}}
\newcommand{\NLO}{{\mathrm{NLO}}}
\newcommand{\PAx}{{\mathrm{PA}}}
\newcommand{\EW}{{\mathrm{EW}}}
\newcommand{\ew}{{\mathrm{EW}}}
\newcommand{\nf}{{\mathrm{nf}}}
\newcommand{\fact}{{\mathrm{fact}}}
\newcommand{\trunc}{{\mathrm{trunc}}}

%codes
\newcommand{\Collier}{{\sc Collier}\xspace}
\newcommand{\HAWKTwo}{{\sc Hawk~2.0}\xspace}
\newcommand{\Recola}{{\sc Recola}\xspace}
\newcommand{\RecolaTwo}{{\sc Recola2}\xspace}
\newcommand{\Prophecy}{{\sc Prophecy4f}\xspace}
\newcommand{\Openloops}{{\sc OpenLoops}\xspace}
\newcommand{\MGNLO}{{\sc MadGraph5\_aMC@NLO}\xspace}
\newcommand{\Gosam}{{\sc GoSam}\xspace}
\newcommand{\FORM}{{\sc FORM}\xspace}
\newcommand{\NLOX}{{\sc NLOX}\xspace}


% SMEFT parameters
\newcommand{\Lop}{\mathcal{O}}
\newcommand{\Lcoeff}{C}

% D-dimensional parameter
\newcommand{\qD}{q}
\newcommand{\DD}{D}
\newcommand{\ND}{N}
\newcommand{\gfour}{\hat{g}}
\newcommand{\qfour}{\hat{q}}
\newcommand{\Dfour}{\hat{D}}
\newcommand{\Nfour}{\hat{N}}
\newcommand{\Afour}{\hat{A}}
\newcommand{\qDmf}{\check{q}}
\newcommand{\DDmf}{\check{D}}
\newcommand{\NDmf}{\check{N}}

% shorthands for HELOGS
\newcommand{\LSC}{\mathrm{LSC}}
\newcommand{\SSC}{\mathrm{SSC}}
\newcommand{\LC}{\mathrm{C}}
\newcommand{\PR}{\mathrm{PR}}
\newcommand{\cew}{C^{\ew}}
\newcommand{\bew}{b^{\ew}}

\newcommand{\qperp}{\mathbf{q}_\perp}

% roman text in equations
\newcommand{\elm}{\text{em}}

\newcommand{\Li}{{\mathrm{Li}}}

% new environments
\newenvironment{myenumerate}%
{\begin{enumerate}[label=(\alph*),leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=2pt plus 1pt minus 1pt,parsep=0pt]}%
{\end{enumerate}}
\newenvironment{myitemize}%
{\begin{itemize}[leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=2pt plus 1pt minus 1pt,parsep=0pt]}%
{\end{itemize}}
\newenvironment{myaitemize}%
{\begin{itemize}[leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=4pt plus 2pt minus 2pt,parsep=0pt]}%
{\end{itemize}}

% new paragraph
\makeatletter
\newcommand\myparagraph{\@startsection{paragraph}{4}{\z@}%
  {-10\p@ \@plus 6\p@ \@minus 3\p@}%
  {3\p@}%
  {\normalfont\itshape}%
}
\makeatother

\newcommand*{\doi}[1]{\href{http://dx.doi.org/#1}{doi: #1}}


%use of align   ={}&
%use of align   & {-x}   if sign

